The completeness-corrected rate of stellar encounters with the Sun from the first Gaia data release

I report on close encounters of stars to the Sun found in the first Gaia data release (GDR1). Combining Gaia astrometry with radial velocities of around 320 000 stars drawn from various catalogues, I integrate orbits in a Galactic potential to identify those stars which pass within a few parsecs. Such encounters could influence the solar system, for example through gravitational perturbations of the Oort cloud. 16 stars are found to come within 2 pc (although a few of these have dubious data). This is fewer than were found in a similar study based on Hipparcos data, even though the present study has many more candidates. This is partly because I reject stars with large radial velocity uncertainties (>10 km/s), and partly because of missing stars in GDR1 (especially at the bright end). The closest encounter found is Gl 710, a K dwarf long-known to come close to the Sun in about 1.3 Myr. The Gaia astrometry predict a much closer passage than pre-Gaia estimates, however: just 16 000 AU (90% confidence interval: 10 000 to 21 000 AU), which will bring this star well within the Oort cloud. Using a simple model for the spatial, velocity, and luminosity distributions of stars, together with an approximation of the observational selection function, I model the incompleteness of this Gaia-based search as a function of the time and distance of closest approach. Applying this to a subset of the observed encounters (excluding duplicates and stars with implausibly large velocities), I estimate the rate of stellar encounters within 5 pc averaged over the past and future 5 Myr to be 545 +/- 59 per Myr. Assuming a quadratic scaling of the rate within some encounter distance (which my model predicts), this corresponds to 87 +/- 9 per My within 2 pc. A more accurate analysis and assessment will be possible with future Gaia data releases.

==> extras.tex <==
%%%%% Old explanation for non-invariance in time of Pmod(tph,dph), and partially dupliate explanation for form of Pmod(tph|dph)

The $P(\tph, \dph)$ distribution is not invariant under translations in the {\em perihelion} time, but this does not mean we are observing at a privileged time.  After all, there is no time evolution of the stellar population in our model, so we would make this same prediction for any time in the past of future.  It is important to realise that these plots show when and where stars {\em which we observe now} will be at perihelion.
(The time axis is not observation time.)
The drop-off at large perihelion times is {\em not} because space is emptied of stars (stars that would then not be available for future generations to observe), but is for the following reason.
In order for a star to encounter at a distance $\dph$ of the Sun, the star must enter a thin
spherical shell (centered on the Sun) of radius $\dph$. The volume of this shell scales as $\dph^2$.
Stars with encounter times far in the future are generally further away now, and the probability that stars enter the shell is smaller the further away they are (because the angular size presented by the shell from the star is smaller). 
% But these encountering stars are also coming from a shell ("outer shell") of radius r, with volume r^2. So if the space density is constant, then more distant stars may have a small chance of hitting the inner shell, but the outer shell is also larger, i.e. more stars. So is the previous argument even relevant? Is it just the next one? If so, then the text I had before may be sufficient and more accurate, which was "It is rather that stars which are currently very distant have encounter times far in the future, and there are relatively few of these, due to the form of P(r)." But I think we need both parts of the argument, because in model33 the space density is essentially constant, yet we still see the rise in P(tph|dph) for smaller tph.
Furthermore, the density of stars at these larger distance is also smaller, because of the form of $P(r)$.
Thus we get a decrease in encountering density for larger perihelion times.
% Andy Gould it not convinced of this argument, because for encounter times up to a few hundred thousand years the encountering stars are all within a few 10s of pc where there is essentially no drop off of density Pmod(r). Maybe he is in principle correct, but because P(r) *is* decreasing for ALL r, we see the effect even at small distances. Plus one can't intuitively say that the gradient is so small at small times that the gradient must be flat. I tested his hypothesis with completeness/model33, which suggests my explanation is correct (see following footnote)
% TODO: Is the following text correct? If so, is it okay?
In some sense the adopted static distance and velocity distributions are not self-consistent, because this velocity distribution would lead to a changing spatial distribution.

%%%%% Table 3 with an extra columns

\item The common objects between this reduced RVcat and ASTcat are identified (using the Tycho IDs). These 98\,714 objects all have -- by construction -- a Tycho ID, TGAS data, positive parallaxes, $|\vr| \leq 750$\,\kms, $\sigvr \leq 10$\,\kms, and {\em would} encounter the Sun within 10\,pc (using the LMA) if they had a radial velocity of 750\,\kms.
The number coming from each RV catalogue is shown in the fourth column of Table \ref{tab:RVcatalogues}.
Of these, 709 have $\dphlin<10$\,pc, now computed using the measured radial velocity. The number per RV catalogue is shown in the fifth column of Table \ref{tab:RVcatalogues}.
Only these objects will be considered in the rest of this paper.
The distribution of the measurements, including their standard deviations and correlations, can be found in \cite{2017IAUS..331..xxxB}.

\begin{table}
\begin{center}
\caption{The number of objects (not unique stars) in the RV catalogues.
The first column gives the catalogue reference number (used in Table \ref{tab:periStats}) and the second column a reference name. 
The third column lists the number of objects with valid Tycho IDs which also have $|\vr|\leq750$\,\kms\ and $\sigvr\leq10$\,\kms. This is approximately the number of objects available for searching for encounters.
The fourth column gives the number which also have TGAS astrometry and positive parallaxes and would encounter the Sun within 10\,pc if they had $|\vr|=750$\,\kms.
The fifth column lists how many of these have $\dphlin < 10$\,pc.
There are duplicate stars between (and even within) the catalogues.
\label{tab:RVcatalogues}}
\begin{tabular}{ r r r r r }
\toprule
cat & name & \#Tycho & \#matched & \#($\dphlin<10$\,pc)\\
\midrule
  1 & RAVE-DR5 & 302\,301  & 60\,706  & 235  \\
  2 & GCS2011 &  13\,547   & 9\,783  & 157  \\
  3 & Pulkovo & 35\,723  & 17\,474 &  233  \\
  4  & Famaey2005 &  6\,047  & 1\,870   & 1 \\
  5  & Web1995 &   414   & 163   & 3  \\
  6  & BB2000 &   648   & 260  &  3  \\
  7 &  Malaroda2012 &   1\,987  &  802  & 12  \\
  8  & Maldonado2010  &  349  &  204  & 32  \\
  9  &  Duflot1997 &   43    & 19  &  0 \\
 10 &  APOGEE2 &  25\,755 &  5\,894  & 31  \\
 11  & Gaia-ESO-DR2   &  159   &  46   & 0  \\
 12 & Galah & 10\,680  & \,493 &   2  \\
\midrule
Total & & 397\,653 & 98\,714 & 709 \\
\bottomrule
\end{tabular}
{\bf Notes:} References and (where used) CDS catalogue numbers for the RV catalogues: (1) \cite{2017AJ....153...75K}; (2) \cite{2011A&A...530A.138C} {\tt J/A+A/530/A138/catalog}; (3) \cite{2006AstL...32..759G} {\tt III/252/table8}; (4) \cite{2005A&A...430..165F} {\tt J/A+A/430/165/tablea1}; (5) \cite{1995A&AS..114..269D} {\tt III/190B}; (6) \cite{2000A&AS..142..217B} {\tt III/213}; (7) \cite{2000A&AS..144....1M} {\tt III/249/catalog}; (8) \cite{2010A&A...521A..12M} {\tt J/A+A/521/A12/table1}; (9) \cite{1997A&AS..124..255F} {\tt J/A+AS/124/255/table1}; (10) \cite{2016arXiv160802013S}; (11) {\tt https://www.gaia-eso.eu}; (12) \cite{2017MNRAS.465.3203M}.
\end{center}
\end{table}

